Studying patched spacetimes for binary black holes

Circumbinary accretion disks have been examined, theoretically, for supermassive and intermediate mass black holes, however, disks for black hole masses in the LIGO regime are poorly understood. Assuming these binaries possess such a disk initially, the question we want to answer is: are they dissipated by outflows or accretion prior to inspiral? To study this problem we propose a novel approach, whereby we consider an approximate, analytic spacetime and solve the geodesic equation for particles in this spacetime so that we can determine the likely fate of particles coming from the accretion disk. Preliminary indications suggest a likelihood of accretion prior to inspiral.

==> bib.tex <==
@article{Alvi:1999cw,
    author = "Alvi, Kashif",
    title = "{An Approximate binary black hole metric}",
    eprint = "gr-qc/9912113",
    archivePrefix = "arXiv",
    doi = "10.1103/PhysRevD.61.124013",
    journal = "Phys. Rev. D",
    volume = "61",
    pages = "124013",
    year = "2000"
}
